Inference for extreme earthquake magnitudes accounting for a time-varying measurement process

Investment in measuring a process more completely or accurately is only useful if these improvements can be utilised during modelling and inference. We consider how improvements to data quality over time can be incorporated when selecting a modelling threshold and in the subsequent inference of an extreme value analysis. Motivated by earthquake catalogues, we consider variable data quality in the form of rounded and incompletely observed data. We develop an approach to select a time-varying modelling threshold that makes best use of the available data, accounting for uncertainty in the magnitude model and for the rounding of observations. We show the benefits of the proposed approach on simulated data and apply the method to a catalogue of earthquakes induced by gas extraction in the Netherlands. This more than doubles the usable catalogue size and greatly increases the precision of high magnitude quantile estimates. This has important consequences for the design and cost of earthquake defences. For the first time, we find compelling data-driven evidence against the applicability of the Gutenberg-Richer law to these earthquakes. Furthermore, our approach to automated threshold selection appears to have much potential for generic applications of extreme value methods.

==> inference_for_extreme_earthquake_magnitudes (arXiv) 2/04_supplementary_figures.tex <==

\section{Supplementary figures}

% Plot of mles and error decomposition for simulation study on the benefits of using a stepped threshold.


\begin{figure}
    \centering
        \includegraphics[width = 0.45\textwidth, page = 1]{sm_figures/supplementary_figures/motivating_example_mle_values.pdf}
        %\qquad \qquad \qquad
         \includegraphics[width = 0.45\textwidth, page = 1]{sm_figures/supplementary_figures/motivating_example_mse_decomposition.pdf}
    \caption{[Left] Plot of maximum likelihood estimates of GPD scale and shape parameters for 1000 simulated catalogues obtained using a conservative, stepped and extended approach. [Right] Plot of mean squared error decomposition for maximum likelihood estimates by each approach. The error is decomposed into squared bias and variance terms for each of the GPD parameters, with variance terms having larger contributions.}
    \label{fig:sim_cat_mse}
\end{figure} 


\begin{figure}
    \centering
    % \includegraphics[width = \textwidth]{figures/flat_threshold_sim/selected_threshold_summary.pdf}
    %
    \includegraphics[width = 0.45 \textwidth, page = 3]{sm_figures/supplementary_figures/selected_threshold_summary_individual_hard.pdf}
    %\qquad \qquad 
    \includegraphics[width = 0.45\textwidth, page = 4]{sm_figures/supplementary_figures/selected_threshold_summary_individual_hard.pdf}
    %
    \caption{Sampling distribution of threshold selection methods for PP-based metrics over 500 simulated catalogues with constant threshold and hard censoring. The true threshold is shown by a dashed red line and the root mean squared error (RMSE) for each method is given in plot titles.}
    %
    \label{fig:flat_threshold_selection_pp_summary}
\end{figure} 


\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{sm_figures/supplementary_figures/groningen_conservative_boot_mles.png}
    %\qquad \qquad \qquad
    \includegraphics[width = 0.45\textwidth]{sm_figures/supplementary_figures/return_levels_conservative.pdf}
    \caption{[left] Bootstrap maximum likelihood estimates for GPD parameters for Groningen magnitudes above 1.45ML assuming GPD (black) and exponential (red) models. [right] Resulting conditional return level plot with return period measured in number of events exceeding 1.45 ML.}
    \label{fig:groningen_mles_and_return_levels_above_145}
\end{figure} 

\vspace{-5cm}
\begin{figure}
    \centering
    % \includegraphics[width = \textwidth]{figures/flat_threshold_sim/selected_threshold_summary.pdf}
    %
    \includegraphics[width = 0.8\textwidth]{sm_figures/supplementary_figures/flat_phased_selection_summary.pdf}
    %
    \caption{Sampling distribution of threshold selection methods for QQ-based (top row) and PP-based (bottom row) metrics over 500 simulated catalogues with constant threshold and phased censoring. The true threshold is shown by a dashed red line and the root mean squared error (RMSE) for each method is given in plot titles.}
    %
    \label{fig:flat_threshold_selection_pp_qq_summary_phased}
\end{figure}  



==> inference_for_extreme_earthquake_magnitudes (arXiv) 2/05_code.tex <==
\section{Code}
An R package is currently under development to implement the methods introduced in this paper. Unpolished R code used for the analyses of the main text can be found at \url{https://github.com/zakvarty/threshold_paper_code}.
